Opportunistic Federated Learning: An Exploration of Egocentric Collaboration for Pervasive Computing Applications

Pervasive computing applications commonly involve user's personal smartphones collecting data to influence application behavior. Applications are often backed by models that learn from the user's experiences to provide personalized and responsive behavior. While models are often pre-trained on massive datasets, federated learning has gained attention for its ability to train globally shared models on users' private data without requiring the users to share their data directly. However, federated learning requires devices to collaborate via a central server, under the assumption that all users desire to learn the same model. We define a new approach, opportunistic federated learning, in which individual devices belonging to different users seek to learn robust models that are personalized to their user's own experiences. However, instead of learning in isolation, these models opportunistically incorporate the learned experiences of other devices they encounter opportunistically. In this paper, we explore the feasibility and limits of such an approach, culminating in a framework that supports encounter-based pairwise collaborative learning. The use of our opportunistic encounter-based learning amplifies the performance of personalized learning while resisting overfitting to encountered data.

==> cj.tex <==
Smartphones, wearable devices, and other computational units ubiquitous in our environment are imbued with increasingly more complex sensing, computational, and communication capabilities. 
These devices are capable of generating (and distributing) vast quantities of data that can be leveraged to build sophisticated machine learning models for a variety of applications, e.g. classification and recommendation. In this work, we explore a new direction that we term {\em pervasive federated learning}, where individual pervasive computing devices cooperate to learn personalized\slee{I think the term `personalized' has been used to indicate that the model is optimized for the (underlying) data distribution of individuals. In our case it would be optimization for some known user requirement. Should we use some other expression? } models informed by both an individual's experience and by the experiences of similar individuals that the device may opportunistically encounter.

{\bf The Setting.} We consider a world where pervasive computing applications aim to learn models that may be used for classification, recommendation, or prediction. The training data is {\em crowdsourced} -- it is generated by a vast set of independent devices. The targeted models are potentially {\em personal}, both with respect to the fact that their outputs may be tailored to an individual (person or device) and to the fact that the training data may be privileged, private, or proprietary. While pervasive computing devices may be vastly heterogeneous in terms of computational, communication, and energy capabilities, for simplicity, we assume two types of devices: (1)~a powerful centralized device (i.e., a cloud system) and (2)~many homogeneous but less powerful edge devices (i.e., smartphones and IoT devices). The devices are capable of communicating with each other; the connectivity graph of the network may range from one representing continual and complete connectivity to one of purely opportunistic encounter-based connectivity.

{\bf Overarching Contributions.} In the long term, we aim to examine a continuum of scenarios that range between two extremes (Figure~\ref{fig:continuum}): at one end, distributed devices learn a single shared global model, while at the other end, each individual participant learns its {\em own} model; in between, models of individual participants are informed by the experiences of others. The field of {\em federated learning} adopts the first extreme, where the shared global model is computed by a single central aggregator using model parameters of the individual nodes (rather than learning directly from the individuals' raw data). At the other extreme, {\em personalized learning} uses a generic model as a foundation and then incorporates a single individual's data to tailor the model to the individual. The continuum shown in Figure~\ref{fig:continuum}\cj{I think there is a very real and important potential for a survey paper here that looks at the existing work that falls on this continuum and could be applied to pervasive computing environments.} considers a spectrum of learning frameworks in which an individual's model can be built by ``mixing-in" information from others' models at varying levels of granularity.

\begin{figure*}[tb]
\includegraphics[width=2\columnwidth]{researchcontinuum}
\caption{\it The continuum of settings to be explored.}\label{fig:continuum}
\end{figure*}

{\bf A First Step.} In this work, we examine the applicability of our vision of {\em pervasive federated learning} to real-world pervasive computing applications.

Characterization of the situations that we aim to address:
\begin{itemize}
    \item distributed personal computing devices that opportunistically encounter one another through wireless interactions
    \item network exchanges have limited capability (in terms of energy, throughput, etc.)
    \item each individual learns its own model of some phenomenon that should be reflective of the data that individual sees\cj{this assumption is what differentiates our goal from that of classical federated learning and puts us in the realm of personalized learning}
    \item the distribution of data that an individual sees is characterized by the raw data items' labels
\end{itemize}

\tocheckCJ{
From here, I'm laying out a research agenda. This is, in my opinion, a rich and long-term research agenda. We need to carve out some specific and concrete thing to work on first.

Variations:
\begin{itemize}
    \item If the distribution of sample labels is the same across all individuals, then they share the goal of learning the same model. This is the operating assumption of classical federated learning.
    \item If the distribution of sample labels differs across individuals, then different individuals will need to learn different models.
    \begin{itemize}
        \item A clustering approach might aim to identify subsets of individuals who have the same distribution and then learn shared models for these clusters. This could also be considered to be equivalent to a classical federated learning approach that considers the ``cluster'' as another feature of the data.
        \item Alternatively, given an opportunistic encounter, an individual might make an opportunistic decision about (1) whether to ``learn'' from the encountered neighbor; (2) what to share in that encounter (raw data or some aspect of the model), which has privacy implications; (3) and how to weight the experiences of the encountered neighbor relative to the individual's own experiences. Aspects that might influence these choices include: (1) how similar the two devices' label distributions are, which could be captured through multiple different metrics; (2) how dissimilar (or similar) were the models that the two devices' ``started'' from (either upon initialization or since they last encountered each other).
        \item Another avenue of investigation is to think about the weighting of the test set that is the target of convergence. An individual might have some labels for which high accuracy is essential, and, for the rest, if the model does well, that's gravy, but the individual doesn't want to sacrifice performance on the ``important'' labels. One could think about this tradeoff as binary or as a continuous scale. And after that ... what if what is important changes over time?
    \end{itemize}
\end{itemize}

Existing work\cj{This is where I need help. I need to better understand what aspects of the above vision are already ``covered'' by the existing work (and in what ways).}

}

\tbc{Pervasive Computing Scenario(s)}

==> evaluation.tex <==

\tocheckSL{To simulate the most realistic settings, we combine mobility data, obtained from levy walk simulation and real-world check-in dataset with benchmark on Raspberry Pi 4.

\subsection{Levy walk}
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.3]{figures/levy_sim.png}
%\caption{Levy walk for 10 episodes \tocheckSL{To be replaced with better pdf version}} 
%\label{fig:levy-sim}
%\end{figure}
Levy Walk is known to simulate human mobility pattern well \cite{rhee2011levy} \cite{rhee2008demystifying} for it's heavy-tail nature, as humans stay at one place and make occasional big jumps to other place rather than consistently walking around. Also, it's proven useful to model
mobile wireless networks \cite{birand2011dynamic}, \cite{hong2008routing}. 

As in \cite{birand2011dynamic}, truncated Levy distribution is used to approximate the distance a device travels and the time it stays at a certain position. Formally,

\begin{equation}
    p(l) \sim \it{T}(\tau, \zeta), l < \tau, 0 < \zeta \leq 2 .
\end{equation}

$\it{T}$ denotes truncated levy distribution where the maximum value of the random variable cannot exceed $\tau$, and 


We created a simulation space with a shape of a square, where devices move around according to Levy Walk. 
To simulate data distribution among devices that is location-specific, we divided the square into 9 quadrants, and devices' local data distribution is determined by which quadrant their initial location is. The simulation is conducted with 45 

\subsection{Simulation}
We train the bootstrap model to the point when it starts overfitting.

\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figures/final.png}
\caption{Example graph for final simulation \tocheckSL{To be replaced with better pdf version(and better result}} 
\label{fig:final-sim}
\end{figure}

\subsection{Discussion}
  as the neural network gets bigger, it gets prone to overfitting, which means that the number of local data would have to increase proportionally
}

==> format.tex <==
%for A4
%\textheight 24.7cm
%\textwidth  16.0cm
% \textheight 9in
% \textwidth 6.5in
\topmargin 0pt
\topmargin  -12pt
%\headheight 15pt
\headsep    4pt
\baselineskip -1pt
\oddsidemargin 0in
\evensidemargin 0in
%\evensidemargin -14pt
%\oddsidemargin -14pt
\itemindent .05in
\labelwidth .0in

\setlength{\itemsep}{-.5in}
\setlength{\parskip}{\smallskipamount}
\makeatletter
\renewcommand{\section}{\@startsection
  {section}% name
  {1}% level
  {0mm}% indent
  {1pt}% beforeskip
  {1pt}% afterskip
  {\large\bfseries}}
\makeatother


\makeatletter
\renewcommand{\subsection}{\@startsection
  {subsection}% name
  {2}% level
  {0mm}% indent
  {1pt}% beforeskip
  {1pt}% afterskip
  {\bfseries}}
\makeatother


\makeatletter
\renewcommand{\subsubsection}{\@startsection
  {subsubsection}% name
  {3}% level
  {0mm}% indent
  {1pt}% beforeskip
  {1pt}% afterskip
  {\itshape}}
\makeatother

\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> motivational_experiments.tex <==
{

\subsubsection{Experiment 1: How does a difference in data distribution affect the benefit of aggregation?}
From a number of works on federated learning\slee{add citations}, it is shown that, in over-parameterized models, even a simple parameter averaging between two models is sufficient to yield a better performance if the data distribution in $\mathcal{D}_1$ and $\mathcal{D}_2$ is iid. Intuitively, if the data distribution is non-iid, model performance is significantly impaired by parameter averaging. In this experiment, we work with a toy example that illustrates a single encounter of two clients to
show that this can be overcome by running multiple rounds of federation, and the necessary number of rounds is dependant on the difference of two data distributions.

Two clients $C_1$ and $C_2$ hold the model $\theta_1$ and $\theta_2$. When they decide to exchange their models, they will run $t \geq 0$ federation rounds ($t = 0$ indicates that the clients only shared the parameters, not running any training after the aggregation). The models are trained from the same randomly initialized model using their local data for some epochs. The two users have been training their models with datasets $\mathcal{D}_1$ and $\mathcal{D}_2$ respectively, which are two different subsets of MNIST dataset. In this scenario, the personalized learning objective of user $C_1$ is to achieve the best accuracy for labels 0 to 4. Distribution of $\mathcal{D}_1$ is identical to this objective, which is only taken from labels from 0 to 4. Now, we look into how similar the data distribution should be in $\mathcal{D}_2$ for $C_1$ to benefit from it. For example, on one extreme, if $\mathcal{D}_2$ is composed of labels from 0 to 4, which is iid to the distribution of $\mathcal{D}_1$, we can expect $C_1$ benefiting from the aggregation. On the other extreme, if $\mathcal{D}_2$ only consisted of labels from 5 to 9, the accuracy on label 0 to 4 will decrease upon aggregation, which is not a desired outcome for $C_1$. 

As the data distribution of $\mathcal{D}_2$ differ from that of $\mathcal{D}_1$, we find that more number of federation rounds is needed to reach a desired accuracy increase of 2\%. We follow the model and hyperparameter settings from \cite{mcmahan2017communication} to provide a meaningful comparison. For models $\theta_1$ and $\theta_2$, we used a fully connected neural network with two hidden layers with 200 units of ReLU activations. The weight for aggregating models is equal for both clients for the simplicity of the experiment. The size of dataset $\mathcal{D}_1$ and $\mathcal{D}_2$ which are used to pretrain the model is 600, and there are no overlapping data points between two clients. Labels, however, overlap between two clients and the overlap decreases in a "sliding window" manner. The offset in the graph indicates how many data points are replaced with a data from different labels.


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/demo_fig_2.pdf}
\caption{The number of federation rounds required to reach 2\% increase in accuracy. Distribution of the opponent's data from which the model is trained deviates from the target model. This result is averaged from 7 experiments.\tocheckSL{This graph will be substituted with lookup table graphs with adding noise.}}
\label{fig:motiv_exp1}
\end{figure}

\subsection{Further Experiments}\cj{To me, these could really come after the description of the approach. They are more a case study of whether our approach is working or not.}\jz{as discussed in the meeting, this will be merged in the Experiments section}
\begin{itemize}
    \item Model a virtual world where there are several groups of agents which have similar datasets and mobility pattern. 
    \item Plug in a real-world training dataset and mobility dataset, and make a semi-simulation. \cite{luo2019real} is a good example for training dataset, as it is non-iid for locations.
\end{itemize}
}

\tocheckCJ{
Additional possible experiments for this section:
\begin{itemize}
    \item Similar to figure 1, but as mentioned in the ``todo'' ... try more randomly subbing in non-iid data. If node 1's training data is (always) comprising labels 0-4, then node 2's training data will be $100-k\%$ labels 0-4, and $k\%$ labels randomly chosen from 5-9. Vary $k$ along the x-axis from 0-100 in, say, 5\% increments. Do multiple runs to generate a smooth trendline.
    \item repeat for target accuracy ranging from $0\%$ to $10\%$ in increments of 1 or 2; do multiple runs to ensure a smooth trendline. We can show multiple lines on the same graph. 
    \item repeat these experiments for multiple data sets
    \item investigate how a node communicates its data distribution after it has done some rounds of federated averaging (how do we ``rebase'' models that have perhaps diverged too far?)
    \item design some experiments to run for when the label distribution of a given node's goal may not be the same as the label distribution of the training data. Ideally, the goal here is to show that the metric should be computed over the goal labels not over the training labels.
\end{itemize}

After this section, the goal is to distill what we've learned into a concrete {\em metric} for comparing the label distribution skews of two nodes that encounter one another. This, combined with a target accuracy improvement, lead to a decision about whether to average or not. Then the meat of the next section is in describing the metric and the middleware for supporting pairwise federated averaging in the needed number of rounds (and stopping when it's ``good enough'').
}



==> research.tex <==
{

% \subsection{Insights}
Agents share models in a given condition. The examples are: physical distance, permission group for sharing models

}

==> scenarios.tex <==
{\begin{itemize}
    \item Mobile Nodes only
    \item Smart City (Static + Mobile nodes)
\end{itemize}
}

==> scope.tex <==
{
Despite its benefits, decentralized federated learning(FL) seems very hard to be realized for its loose guarantee for convergence. In this paper, we investigate techniques to make decentralized deep learning feasible, especially in the domain of pervasive computing. We define rather peculiar goal for our decentralized FL. The conventional centralized federated learning model aims to find a global model that performs the best to the underlying data distribution of the whole dataset. In contrast, We argue that this is not necessary nor desirable in the context of decentralized FL\slee{But what about the case where it is desirable? For example, if the user moves to a new area where data distribution is different.}. First, we identify the shortcomings of naive approach to decentralized learning compared to centralized FL with experiments. Second, we show how we can overcome this with \textit{version thresholding}. Third, we evaluate our scheme with benchmark dataset and simulation with real-world dataset and mobility models in both iid and non-iid dataset. Furthermore, we conduct experiment in two cases of non-iidness, \textit{feature distribution skew} and \textit{label distribution skew}.
\begin{itemize}
    \item Non-iidness characterized by mobility patterns: If dataset of nodes are dependant to the mobility pattern, we can exploit this to enhance personalization within virtual clusters. Decentralized FL in this case can be seen as FL in loosely clustered nodes.
    \item Non-iidness that harms decentralized FL: We talk about techniques to mitigate non-iidness of data.
\end{itemize}

}

==> systemmodel.tex <==
{
\tocheckSL{
\subsection{Pervasive Federated Learning vs. Existing Approaches}
The premises of works on federated learning or decentralized learning is that the aggregator has view of a group of a sufficient number of clients that will consequently benefit to the convergence of global model. The view has to be maintained in some time window, e.g., at a certain time of a day\cite{bonawitz2019towards}, or the client has to be powerful enough to keep a history to build a view over time\cite{vanhaesebrouck2017decentralized}. However, this is very hard to happen in pervasive computing environments, as the devices could be scattered not to mention their restricted computational resources. Even if we assume a domain with densely populated devices, the bandwidth constraints prevents us from obtaining updates from them in a reasonable time window. 

Given a client that aggregates parameters from its neighbors, a single aggregation with a model with bad local minima could yield a catastrophic result to the model's performance. This can't be tolerated in the application point of view, where the deployed model could be utilized by the user at any time. We investigate how to dynamically optimize the model from a single client's point of view, only opportunistically integrating updates from other clients. This is in contrast to classic federated learning where the objective is to minimize the loss of a global model, regardless of how the individual models distributed across devices perform during the process. Similarly, existing works on decentralized learning in peer-to-peer environment\cite{iutzeler2013asynchronous, colin2016gossip} concerns solving a consensus problem to find a global solution. 

In existing works\cite{jiang2019improving, vanhaesebrouck2017decentralized}\slee{*put different related works here}, what is generally referred to as {\em personalization} concerns techniques to optimize clients' model against its own dataset(or underlying data distribution of it), while training a global model. In this paper, we focus on optimizing the model against given requirements. ...\slee{some justification of why this happens frequently in pervasive settings.} For instance, if a client was to personalize its model to a given data distribution, chances are that it doesn't even have dataset to validate its own model.
}

\subsection{Model Description}
In pervasive FL, we assume a set of $N$ devices $\mathcal{C} = \{C_1, ... ,C_N\}$ which hold data $\mathcal{D} = \{D_1, ... ,D_N\}$ and on-device deep learning model $\Theta = \{\theta_1, ... ,\theta_N\}$. The devices don't have any prior knowledge about the existence of other devices. One device can ask another for \textit{training delegation} when they're in close proximity.

\begin{equation}
    \theta^{(t+1)}_i = \lambda\theta^{t}_i + (1-\lambda)\theta^{t}_j
\end{equation}

\begin{equation}
    \min_{\theta_i}(\mathcal{L}_i(\theta_i^{t+1}; \mathcal{D}_{req}) - \mathcal{L}_i(\theta_i^{t}; \mathcal{D}_{req}))
\end{equation}

Here, we assumed a global clock that increments whenever there's an encounter between clients for the convenience of discussion.

\begin{algorithm}[tb]
\caption{Federation}
\label{alg:req}
\DontPrintSemicolon

\end{algorithm}
}
